Tensor-Based Receivers for the Bistatic Sensing and Communication Scenario

We propose receivers for bistatic sensing and communication that exploit a tensor modeling of the received signals. We consider a hybrid scenario where the sensing link knows the transmitted data to estimate the target parameters while the communication link operates semi-blindly in a direct data decoding approach without channel knowledge. We show that the signals received at the sensing receiver and communication receiver follow PARATUCK and PARAFAC tensor models, respectively. These models are exploited to obtain accurate estimates of the target parameters (at the sensing receiver) and the transmitted symbols and channels (at the user equipment). We discuss uniqueness conditions and provide some simulation results to evaluate the performance of the proposed receivers. Our experiments show that the sensing parameters are well estimated at moderate signal-to-noise ratio (SNR) while keeping good symbol error rate (SER) and channel normalized mean square error (NMSE) results for the communication link.

==> biblio.tex <==
\begin{thebibliography}{10}
\bibliographystyle{unsrt}
\expandafter\ifx\csname url\endcsname\relax
  \def\url#1{\texttt{#1}}\fi
\expandafter\ifx\csname urlprefix\endcsname\relax\def\urlprefix{URL }\fi

	\bibitem{Liu:20} F. Liu, C. Masouros, A. Petropulu, H. Griffiths \& L. Hanzo. ``Joint radar and communication design: Applications, state-of-the-art, and the road ahead.'' in IEEE Transactions on Communications, vol. 68, no. 6, pp. 3834–3862, 2020.

	\bibitem{Lu:2024} S. Lu et al., "Integrated Sensing and Communications: Recent Advances and Ten Open Challenges," in IEEE Internet of Things Journal, vol. 11, no. 11, pp. 19094-19120, 1 June1, 2024.

	\bibitem{3GPP:TS22.137} 3GPP TS 22.137, 3rd Generation Partnership Project; Technical Specification Group TSG SA; Service requirements for Integrated Sensing and Communication; Stage 1 (Release 19).

	\bibitem{3GPP:TS22.837} 3GPP TS 22.837, 3rd Generation Partnership Project; Technical Specification Group TSG SA; Feasibility Study on Integrated Sensing and Communication (Release 19).

	\bibitem{Xiong:2023} Y. Xiong, F. Liu, Y. Cui, W. Yuan, T. X. Han and G. Caire, "On the Fundamental Tradeoff of Integrated Sensing and Communications Under Gaussian Channels," in IEEE Transactions on Information Theory, vol. 69, no. 9, pp. 5723-5751, Sept. 2023.

	\bibitem{Emil:book24} E. Bj\"{o}rnson and \"{O}. Demir. Introduction to Multiple Antenna Communications and Reconfigurable Surfaces. Boston Delft: Now Publishers, 2024.

	\bibitem{Leandro:TSP14} L. R. Ximenes, G. Favier, A. L. F. de Almeida and Y. C. B. Silva, ``PARAFAC-PARATUCK Semi-Blind Receivers for Two-Hop Cooperative MIMO Relay Systems,'' in IEEE Transactions on Signal Processing, vol. 62, no. 14, pp. 3604-3615, July, 2014.

	\bibitem{Walter:SPL:17} W. C. Freitas Jr., G. Favier and A. L. F. de Almeida, "Sequential Closed-Form Semiblind Receiver for Space-Time Coded Multihop Relaying Systems," in IEEE Signal Processing Letters, vol. 24, no. 12, pp. 1773-1777, Dec. 2017.

	\bibitem{Gilderlan:21} G. T. de Ara\'{u}jo, A. L. F. de Almeida and R. Boyer, "Channel Estimation for Intelligent Reflecting Surface Assisted MIMO Systems: A Tensor Modeling Approach," in IEEE Journal of Selected Topics in Signal Processing, vol. 15, no. 3, pp. 789-802, April 2021.

	\bibitem{Zhang:24} R. Zhang et al. ``Integrated Sensing and Communication With Massive MIMO: A Unified Tensor Approach for Channel and Target Parameter Estimation.'' IEEE Transactions on Wireless Communications 23 (2024): 8571-8587.

	\bibitem{Du:24} J.Du, Y. Cheng, L. Jin, S. Li, and F. Gao. ``Nested Tensor-Based Integrated Sensing and Communication in RIS-Assisted THz MIMO Systems.'' Trans. Sig. Proc. 72 (2024), 1141–1157.

	\bibitem{Harshman:96} R. A. Harshman and M. E. Lundy, ``Uniqueness proof for a family
of models sharing features of tuckers three-mode factor analysis and
PARAFAC/CANDECOMP,'' Psychometrika, vol. 61, Mar. 1996, pp. 133–154.

	\bibitem{Bro:98} R. Bro, ``Multi- way analysis in the food industry: Models, algorithms
\& applications,'' Ph.D. dissertation, Univ. Amsterdam, Amsterdam, The
Netherlands, Nov. 1998.

	\bibitem{Ferrer:09} A. L. F. de Almeida, G. Favier and Jo\~{a}o C.M. Mota, ``
Space–time spreading–multiplexing for MIMO wireless communication systems using the PARATUCK-2 tensor model,'' Signal Processing, Volume 89, Issue 11,
2009, Pages 2103-2116.

	\bibitem{Gil:23} G. T. de Ara\'{u}jo, A. L. F. de Almeida, R. Boyer and G. Fodor, ``Semi-Blind Joint Channel and Symbol Estimation for IRS-Assisted MIMO Systems,'' in IEEE Transactions on Signal Processing, vol. 71, pp. 1184-1199, 2023.

	\bibitem{Comon2009} P. Comon, X. Luciani, and A. L. F. de Almeida, ``Tensor decompositions, alternating least squares and other tales,'' Journal of Chemometrics: A Journal of the Chemometrics Society, vol. 23, no. 7-8, pp. 393–405, 2009.

	\bibitem{Favier:bookv2} G. Favier. Matrix and Tensor Decompositions in Signal Processing, Volume 2. John Wiley \& Sons, 2021.

	\bibitem{Favier:PT2} G. Favier and A. L. F. de Almeida, ``Overview of constrained PARAFAC models,'' EURASIP J. Adv. Signal Process. 2014, 142 (2014).

	\bibitem{Freitas:2018} W. C. Freitas Jr., G. Favier and A. L. F. de Almeida, ``Generalized Khatri-Rao and Kronecker space-time coding for MIMO relay systems with closed-form semi-blind receivers,'' Signal Processing, Volume 151, 2018, Pages 19-31, 2018.

	\bibitem{Kibangou:20109} A. Y. Kibangou, G. Favier, ``Non-iterative solution for PARAFAC with a Toeplitz matrix factor,'' in: Proceedings of the Seventeenth European Signal Processing Conference, pp. 691–695, 2009.

	\bibitem{Couras:2023} M.F.K.B. Couras, P.H.U. de Pinho, G. Favier, V. Zarzoso, A.L.F. de Almeida, J.P.J. da Costa, ``Semi-blind receivers based on a coupled nested Tucker-PARAFAC model for dual-polarized MIMO systems using combined TST and MSMKron codings'', Digital Signal Processing, Volume 137, 2023.
\end{thebibliography}



==> biblio_new.tex <==
\begin{thebibliography}{100}

	\bibitem{3GPP:TS22.837} 3GPP TS 22.837, 3rd Generation Partnership Project; Technical Specification Group TSG SA; Feasibility Study on Integrated Sensing and Communication (Release 19).

	\bibitem{3GPP:TS22.137} 3GPP TS 22.137, 3rd Generation Partnership Project; Technical Specification Group TSG SA; Service requirements for Integrated Sensing and Communication; Stage 1 (Release 19).

	\bibitem{Liu:20} F. Liu, C. Masouros, A. Petropulu, H. Griffiths \& L. Hanzo. ``Joint radar and communication design: Applications, state-of-the-art, and the road ahead.'' in IEEE Transactions on Communications, vol. 68, no. 6, pp. 38343862, 2020.

	\bibitem{Emil:book24} E. Bj\"{o}rnson and \"{O}. Demir. Introduction to Multiple Antenna Communications and Reconfigurable Surfaces. Boston Delft: Now Publishers, 2024.

	\bibitem{Xiong:2023} Y. Xiong, F. Liu, Y. Cui, W. Yuan, T. X. Han and G. Caire, "On the Fundamental Tradeoff of Integrated Sensing and Communications Under Gaussian Channels," in IEEE Transactions on Information Theory, vol. 69, no. 9, pp. 5723-5751, Sept. 2023.

	\bibitem{Leandro:TSP14} L. R. Ximenes, G. Favier, A. L. F. de Almeida and Y. C. B. Silva, ``PARAFAC-PARATUCK Semi-Blind Receivers for Two-Hop Cooperative MIMO Relay Systems,'' in IEEE Transactions on Signal Processing, vol. 62, no. 14, pp. 3604-3615, July, 2014.

	\bibitem{Walter:SPL:17} W. C. Freitas Jr., G. Favier and A. L. F. de Almeida, "Sequential Closed-Form Semiblind Receiver for Space-Time Coded Multihop Relaying Systems," in IEEE Signal Processing Letters, vol. 24, no. 12, pp. 1773-1777, Dec. 2017.

	\bibitem{Gilderlan:21} G. T. de Ara\'{u}jo, A. L. F. de Almeida and R. Boyer, "Channel Estimation for Intelligent Reflecting Surface Assisted MIMO Systems: A Tensor Modeling Approach," in IEEE Journal of Selected Topics in Signal Processing, vol. 15, no. 3, pp. 789-802, April 2021.

	\bibitem{Favier:PT2} G. Favier and A. L. F. de Almeida, ``Overview of constrained PARAFAC models,'' EURASIP J. Adv. Signal Process. 2014, 142 (2014).

	\bibitem{Favier:bookv2} G. Favier. Matrix and Tensor Decompositions in Signal Processing, Volume 2. John Wiley \& Sons, 2021.

	\bibitem{Harshman:96} R. A. Harshman and M. E. Lundy, ``Uniqueness proof for a family
of models sharing features of tuckers three-mode factor analysis and
PARAFAC/CANDECOMP,'' Psychometrika, vol. 61, Mar. 1996, pp. 133154.

	\bibitem{Bro:98} R. Bro, ``Multi- way analysis in the food industry: Models, algorithms
\& applications,'' Ph.D. dissertation, Univ. Amsterdam, Amsterdam, The
Netherlands, Nov. 1998.

	\bibitem{Ferrer:09} A. L. F. de Almeida, G. Favier and Jo\~{a}o C.M. Mota, ``
Spacetime spreadingmultiplexing for MIMO wireless communication systems using the PARATUCK-2 tensor model,'' Signal Processing, Volume 89, Issue 11,
2009, Pages 2103-2116.

	\bibitem{Gil:23} G. T. de Ara\'{u}jo, A. L. F. de Almeida, R. Boyer and G. Fodor, ``Semi-Blind Joint Channel and Symbol Estimation for IRS-Assisted MIMO Systems,'' in IEEE Transactions on Signal Processing, vol. 71, pp. 1184-1199, 2023.

	\bibitem{Zhang:24} R. Zhang et al. ``Integrated Sensing and Communication With Massive MIMO: A Unified Tensor Approach for Channel and Target Parameter Estimation.'' IEEE Transactions on Wireless Communications 23 (2024): 8571-8587.

	\bibitem{Du:24} J.Du, Y. Cheng, L. Jin, S. Li, and F. Gao. ``Nested Tensor-Based Integrated Sensing and Communication in RIS-Assisted THz MIMO Systems.'' Trans. Sig. Proc. 72 (2024), 11411157.

	\bibitem{Comon2009} P. Comon, X. Luciani, and A. L. F. de Almeida, ``Tensor decompositions, alternating least squares and other tales,'' Journal of Chemometrics: A Journal of the Chemometrics Society, vol. 23, no. 7-8, pp. 393405, 2009.

	\bibitem{Couras:2023} M.F.K.B. Couras, P.H.U. de Pinho, G. Favier, V. Zarzoso, A.L.F. de Almeida, J.P.J. da Costa, ``Semi-blind receivers based on a coupled nested Tucker-PARAFAC model for dual-polarized MIMO systems using combined TST and MSMKron codings'', Digital Signal Processing, Volume 137, 2023.

	\bibitem{Lu:2024} S. Lu et al., "Integrated Sensing and Communications: Recent Advances and Ten Open Challenges," in IEEE Internet of Things Journal, vol. 11, no. 11, pp. 19094-19120, 1 June1, 2024.

	\bibitem{Freitas:2018} W. C. Freitas Jr., G. Favier and A. L. F. de Almeida, ``Generalized Khatri-Rao and Kronecker space-time coding for MIMO relay systems with closed-form semi-blind receivers,'' Signal Processing, Volume 151, 2018, Pages 19-31, 2018.

	\bibitem{Kibangou:20109} A. Y. Kibangou, G. Favier, ``Non-iterative solution for PARAFAC with a Toeplitz matrix factor,'' in: Proceedings of the Seventeenth European Signal Processing Conference, pp. 691695, 2009.


\end{thebibliography}

%%%%% CLEAR DOUBLE PAGE!
\newpage{\pagestyle{empty}\cleardoublepage}
